The Iterative Optimal Brain Surgeon: Faster Sparse Recovery by Leveraging Second-Order Information

The rising footprint of machine learning has led to a focus on imposing \emph{model sparsity} as a means of reducing computational and memory costs. For deep neural networks (DNNs), the state-of-the-art accuracy-vs-sparsity is achieved by heuristics inspired by the classical Optimal Brain Surgeon (OBS) framework~\citep{lecun90brain, hassibi1992second, hassibi1993optimal}, which leverages loss curvature information to make better pruning decisions. Yet, these results still lack a solid theoretical understanding, and it is unclear whether they can be improved by leveraging connections to the wealth of work on sparse recovery algorithms. In this paper, we draw new connections between these two areas and present new sparse recovery algorithms inspired by the OBS framework that comes with theoretical guarantees under reasonable assumptions and have strong practical performance. Specifically, our work starts from the observation that we can leverage curvature information in OBS-like fashion upon the projection step of classic iterative sparse recovery algorithms such as IHT. We show for the first time that this leads both to improved convergence bounds under standard assumptions. Furthermore, we present extensions of this approach to the practical task of obtaining accurate sparse DNNs, and validate it experimentally at scale for Transformer-based models on vision and language tasks.

==> macros.tex <==

% Recommended, but optional, packages for figures and better typesetting:
\RequirePackage{xcolor}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subcaption}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{caption}
\usepackage{comment}


% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2024} with \usepackage[nohyperref]{icml2024} above.
% \usepackage{hyperref}
\graphicspath{{../figures/}}


% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}


% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{algorithm,algorithmic}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}[theorem]{Corollary}
% \theoremstyle{definition}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{assumption}[theorem]{Assumption}
% \theoremstyle{remark}
% \newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}

\usepackage{thm-restate}
\usepackage{empheq}
\usepackage{authblk}
\usepackage{color}
\definecolor{darkgreen}{rgb}{0.0,0.5,0.0}
\newcommand{\purple}{\color{purple}}
\newcommand{\teal}{\color{teal}}
% \usepackage[pagebackref]{hyperref}
% \hypersetup{
% 	colorlinks=true,        % false: boxed links; true: colored links
% 	linkcolor=blue,         % color of internal links
% 	filecolor=magenta,
% 	citecolor=darkgreen,         % color of links to bibliography
% 	urlcolor=blue           % color of external links
% }
% \renewcommand*{\backrefalt}[4]{%
%     \ifcase #1 \footnotesize{(Not cited.)}%
%     \or        \footnotesize{(Cited on page~#2)}%
%     \else      \footnotesize{(Cited on pages~#2)}%
%     \fi}
% if you use cleveref..
% \usepackage[capitalize,noabbrev]{cleveref}
% cleveref must be loaded after hyperref!.

\usepackage{thm-restate}

\newcommand{\squeeze}{\textstyle}
\newcommand{\eqdef}{\mathrel{\mathop:}=}

==> rebuttal.tex <==
\section*{Extra experiments results}

\begin{table}[h!t]
\caption{Performance of I-OBS on Llama-2-7b}
\centering
\begin{tabular}{cc}
\toprule
\textbf{Iterations} & \textbf{MMLU(5-shot)}  \\
\midrule
0 (dense)  &     0.4584 \\
1          &     0.3878 \\   
2          &    \textbf{0.3950} \\
3          &     0.3932 \\
4          &     0.3943 \\
5          &     0.3946 \\
6          &     0.3929 \\
7          &     0.3919 \\
8          &     0.3893 \\
9          &     0.3903 \\
10         &     0.3863 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h!t]
\caption{Performance of I-OBS on Llama-3-8B}
\centering
\begin{tabular}{cc}
\toprule
\textbf{Iterations} & \textbf{MMLU(5-shot)}  \\
\midrule
  0 (dense)  &      0.6525  \\   
  1          &      0.5476   \\ 
  2          &      0.5577   \\  
  3          &      0.5582   \\  
  4          &    \textbf{0.5605} \\  
  5          &      0.5553   \\  
  6          &      0.5521   \\  
  7          &      0.5444   \\  
  8          &      0.5449   \\  
  9          &      0.5403   \\  
  10         &      0.5375   \\  
\bottomrule
\end{tabular}
\end{table}



\begin{table}[h!t]
    \caption{Comparison of I-OBS and CBS  at different sparsity levels}
    \centering
\begin{tabular}{ccc}
    \toprule
    \textbf{sparsity} & \textbf{I-OBS} & \textbf{CBS} \\
    \midrule
    30\% &         71.6  & \textbf{71.88} \\
    40\% &         71.3  & \textbf{71.45} \\
    50\% & \textbf{70.6} &         70.21  \\
    60\% & \textbf{68.4} &         66.37  \\
    70\% & \textbf{60.7} &         55.11  \\
    80\% & \textbf{27.9} &         16.38  \\

    % 30\% & 71.6 & 71.88 \\
    % 40\% & 71.3 & 71.45 \\
    % 50\% & 70.6 & 70.21 \\
    % 60\% & 68.4 & 66.37 \\
    % 70\% & 60.7 & 55.11 \\
    % 80\% & 27.9 & 16.38 \\
    \midrule
    0\% (dense) & 71.95\% & \\
    \bottomrule
\end{tabular}
\end{table}


